Isospectral hyperbolic surfaces have matching geodesics

We show that if two closed hyperbolic surfaces (not necessarily orientable or even connected) have the same Laplace spectrum, then for every length they have the same number of orientation-preserving geodesics and the same number of orientation-reversing geodesics. Restricted to orientable surfaces, this result reduces to Huber's theorem of 1959. Appropriately generalized, it extends to hyperbolic 2-orbifolds (possibly disconnected). We give examples showing that it fails for disconnected flat 2-orbifolds.

==> verso_dot_bib <==
@incollection {bb:selberg,
   AUTHOR = {B{\'e}rard-Bergery, Lionel},
    TITLE = {Laplacien et g\'eod\'esiques ferm\'ees sur les formes d'espace
             hyperbolique compactes},
 BOOKTITLE = {S\'eminaire Bourbaki, 24\`eme ann\'ee (1971/1972), Exp. No.
             406},
    PAGES = {107--122. Lecture Notes in Math., Vol. 317},
 PUBLISHER = {Springer},
  ADDRESS = {Berlin},
     YEAR = {1973},
  MRCLASS = {53C20 (58G99)},
 MRNUMBER = {MR0420504 (54 \#8518)},
MRREVIEWER = {Midori Goto},
ZBL={0261.53034}
}

@book {buser:book,
   AUTHOR = {Buser, Peter},
    TITLE = {Geometry and spectra of compact {R}iemann surfaces},
   SERIES = {Progress in Mathematics},
   VOLUME = {106},
 PUBLISHER = {Birkh\"auser Boston Inc.},
  ADDRESS = {Boston, MA},
     YEAR = {1992},
    PAGES = {xiv+454},
     ISBN = {0-8176-3406-1},
  MRCLASS = {58G25 (30F99)},
 MRNUMBER = {MR1183224 (93g:58149)},
MRREVIEWER = {Robert Brooks},
ZBL={0770.53001}
}

@book {chavel:eigen,
   AUTHOR = {Chavel, Isaac},
    TITLE = {Eigenvalues in {R}iemannian geometry},
   SERIES = {Pure and Applied Mathematics},
   VOLUME = {115},
     NOTE = {Including a chapter by Burton Randol,
             With an appendix by Jozef Dodziuk},
 PUBLISHER = {Academic Press Inc.},
  ADDRESS = {Orlando, FL},
     YEAR = {1984},
    PAGES = {xiv+362},
     ISBN = {0-12-170640-0},
  MRCLASS = {58G25 (35P99 53C20)},
 MRNUMBER = {MR768584 (86g:58140)},
MRREVIEWER = {G{\'e}rard Besson},
ZBL={0551.53001}
}

@incollection {conway:orbifold,
   AUTHOR = {Conway, J. H.},
    TITLE = {The orbifold notation for surface groups},
 BOOKTITLE = {Groups, combinatorics \& geometry (Durham, 1990)},
   SERIES = {London Math. Soc. Lecture Note Ser.},
   VOLUME = {165},
    PAGES = {438--447},
 PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1992},
  MRCLASS = {57M50 (20F32 57M60)},
 MRNUMBER = {MR1200280 (94a:57025)},
MRREVIEWER = {Denis Sjerve},
ZBL={0835.20048}
}

@article {doylerossetti:cosmic,
   AUTHOR = {Doyle, Peter G. and Rossetti, Juan Pablo},
    TITLE = {Tetra and {D}idi, the cosmic spectral twins},
  JOURNAL = {Geom. Topol.},
 FJOURNAL = {Geometry and Topology},
   VOLUME = {8},
     YEAR = {2004},
    PAGES = {1227--1242 (electronic)},
     ISSN = {1465-3060},
  MRCLASS = {58J53 (11F72 57M50 57N15)},
 MRNUMBER = {MR2087082 (2005j:58046)},
MRREVIEWER = {Dorothee Schueth},
ZBL={1091.58021}
}

@article {gangolli:selberg,
   AUTHOR = {Gangolli, Ramesh},
    TITLE = {The length spectra of some compact manifolds of negative
             curvature},
  JOURNAL = {J. Differential Geom.},
 FJOURNAL = {Journal of Differential Geometry},
   VOLUME = {12},
     YEAR = {1977},
   NUMBER = {3},
    PAGES = {403--424},
     ISSN = {0022-040X},
  MRCLASS = {58G99 (10D15)},
 MRNUMBER = {MR0650997 (58 \#31311)},
ZBL={0365.53016}
}

@article {huber:selbergI,
   AUTHOR = {Huber, Heinz},
    TITLE = {Zur analytischen {T}heorie hyperbolischen {R}aumformen und
             {B}ewegungsgruppen},
  JOURNAL = {Math. Ann.},
 FJOURNAL = {Mathematische Annalen},
   VOLUME = {138},
     YEAR = {1959},
    PAGES = {1--26},
     ISSN = {0025-5831},
  MRCLASS = {30.00},
 MRNUMBER = {MR0109212 (22 \#99)},
MRREVIEWER = {J. Lehner},
ZBL={0089.06101}
}

@article {phillipssarnak:PGT,
   AUTHOR = {Phillips, Ralph and Sarnak, Peter},
    TITLE = {Geodesics in homology classes},
  JOURNAL = {Duke Math. J.},
 FJOURNAL = {Duke Mathematical Journal},
   VOLUME = {55},
     YEAR = {1987},
   NUMBER = {2},
    PAGES = {287--297},
     ISSN = {0012-7094},
    CODEN = {DUMJAO},
  MRCLASS = {58F17 (11F72 58F18)},
 MRNUMBER = {MR894581 (88g:58151)},
MRREVIEWER = {Midori Goto},
ZBL={0642.53050}
}

@article {sunada:method,
   AUTHOR = {Sunada, Toshikazu},
    TITLE = {Riemannian coverings and isospectral manifolds},
  JOURNAL = {Ann. of Math. (2)},
 FJOURNAL = {Annals of Mathematics. Second Series},
   VOLUME = {121},
     YEAR = {1985},
   NUMBER = {1},
    PAGES = {169--186},
     ISSN = {0003-486X},
    CODEN = {ANMAAH},
  MRCLASS = {58G25 (11F72 53C20 57M99)},
 MRNUMBER = {MR782558 (86h:58141)},
MRREVIEWER = {Scott Wolpert},
ZBL={0585.58047}
}

@article {vigneras:isospectral,
   AUTHOR = {Vign{\'e}ras, Marie-France},
    TITLE = {Vari\'et\'es riemanniennes isospectrales et non
             isom\'etriques},
  JOURNAL = {Ann. of Math. (2)},
 FJOURNAL = {Annals of Mathematics. Second Series},
   VOLUME = {112},
     YEAR = {1980},
   NUMBER = {1},
    PAGES = {21--32},
     ISSN = {0003-486X},
    CODEN = {ANMAAH},
  MRCLASS = {58G25 (10J25 12A70)},
 MRNUMBER = {MR584073 (82b:58102)},
MRREVIEWER = {P. Wintgen},
ZBL={0445.53026}
}

@misc{drydenfinite,
title = {{Isospectral Finiteness of Hyperbolic Orbisurfaces}},
author = {Emily B. Dryden},
year="2004",
eprint = {arXiv:math.SP/0411290}}

@misc{drydenstrohmaier,
title = {{Huber's theorem for hyperbolic orbisurfaces}},
author = {Emily B. Dryden and Alexander Strohmaier},
year="2005",
eprint = {arXiv:math.SP/0504571}}

@misc{drydenetal,
title="Asymptotic expansion of the heat kernel for orbifolds",
author="Emily B. Dryden and Carolyn S. Gordon and Sarah J. Greenwald",
year="2008"
}

